Black holes and solution generating techniques

Multi-black hole solutions play a relevant role both from the theoretical and the phenomenological point of view. In this Thesis, we construct some regular multi-black hole spacetimes in pure Einstein's General Relativity with the aid of solution generating techniques. We begin with a perspective on the history of solution generating techniques, and then we explain in detail the Ernst formalism and the inverse scattering method. These are the techniques that are applied in the rest of the Thesis. Subsequently, we construct multi-black hole solutions embedded in an external gravitational field: it is possible to obtain an equilibrium configuration in many interesting cases, like a collection of collinear static black holes or a chain of accelerating black holes, by choosing appropriately the multipole parameters of the field. Then, we consider the expanding bubbles of nothing as a background for multi-black hole and black ring solutions. The expanding behaviour of the bubbles provides the force necessary to balance the gravitational attraction among the black holes, and hence to reach the equilibrium. Finally, we construct a solution that represents a black hole embedded in a "swirling" universe, which describes a spacetime whirlpool. Moreover, we discuss the possibility of implementing the swirling background in order to enforce the spin-spin configuration, and reach an equilibrium configuration in a double-Kerr spacetime.

==> Acknowledgments.tex <==
\chapter*{Acknowledgments}
\thispagestyle{plain}

...
